WARP: A ICN architecture for social data

Social network companies maintain complete visibility and ownership of the data they store. However users should be able to maintain full control over their content. For this purpose, we propose WARP, an architecture based upon Information-Centric Networking (ICN) designs, which expands the scope of the ICN architecture beyond media distribution, to provide data control in social networks. The benefit of our solution lies in the lightweight nature of the protocol and in its layered design. With WARP, data distribution and access policies are enforced on the user side. Data can still be replicated in an ICN fashion but we introduce control channels, named \textit{thread updates}, which ensures that the access to the data is always updated to the latest control policy. WARP decentralizes the social network but still offers APIs so that social network providers can build products and business models on top of WARP. Social applications run directly on the user's device and store their data on the user's \textit{butler} that takes care of encryption and distribution. Moreover, users can still rely on third parties to have high-availability without renouncing their privacy.

==> algorithms_prot.tex <==
\begin{algorithm}[h!]
\begin{minipage}{\linewidth}
\caption{Euclids algorithm}\label{euclid}
\begin{algorithmic}[1]
\Procedure{Euclid}{$a,b$}\Comment{The g.c.d. of a and b}
\State $r\gets a\bmod b$
\While{$r\not=0$}\Comment{We have the answer if r is 0}
\State $a\gets b$
\State $b\gets r$
\State $r\gets a\bmod b$
\EndWhile\label{euclidendwhile}
\State \textbf{return} $b$\Comment{The gcd is b}
\EndProcedure
\end{algorithmic}
\end{minipage}
\end{algorithm}
\begin{algorithm}[h!]
\begin{minipage}{\linewidth}
\caption{Euclids algorithm}\label{euclid}
\begin{algorithmic}[1]
\Procedure{Euclid}{$a,b$}\Comment{The g.c.d. of a and b}
\State $r\gets a\bmod b$
\While{$r\not=0$}\Comment{We have the answer if r is 0}
\State $a\gets b$
\State $b\gets r$
\State $r\gets a\bmod b$
\EndWhile\label{euclidendwhile}
\State \textbf{return} $b$\Comment{The gcd is b}
\EndProcedure
\end{algorithmic}
\end{minipage}
\end{algorithm}



==> app_img.tex <==
\begin{figure*}[t!]
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=\linewidth]{img/layers.jpg}
\subcaption{}
\label{fig:figure2}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=\linewidth]{img/placeholder.jpg}
\subcaption{}
\label{fig:figure1}
\end{minipage}
\caption{{\scriptsize }}
\end{figure*}

==> application.tex <==
\section{Applications}
Being constrained with the number of pages, we cannot give an extensive discussion on WARP's API although in Fig \ref{fig:archcon} we outline the content design of Facebook-like timeline, the pictures show how easily the timeline can be embedded into a WARP's feed to notify the creation of new data objects. The index of the application maintains a reference to the latest portion of the feed so that an application can always request only the latest news.
Content is generated by social applications that store it into the butler's DB via APIs, for this purpose WARP APIs offer all the CRUD\footnote{common acronym for Create, Read, Update and Delete} functionalities. Additionally, the application is allowed to compile the index file of its folder, create feeds and map DB content into network objects. Moreover, they can subscribe to be notified whenever a NOTIFY message arrives to the butler.   
Social applications that run directly on the butler can be prevented from accessing to the network and distribute unencrypted data of the user, their mobile instances however could maliciously read the content storage and transfer the data somewhere else. In order to prevent this problem mobile instances can only read from the database the data that they produced.

%A summary of WARP API is:
%\textbf{Create/Remove Feed} Notifies the network layer to create or delete a new feed \\
%\textbf{Append to Feed} Appends a network object to a feed\\
%\textbf{Remove Feed Segment} removes a segment from a feed\\
%\textbf{Publish/Unpublish Content} map/unmap a db record to/from a network object\\
%\textbf{Add new Feed entry} Adds a new entry to the feed \\
%\textbf{Notify Content} notify another butler about the existence of another content\\
%\textbf{Create Thread} Creates a new thread\\
%\textbf{Bind/Unbind Thread} Binds a network object to a thread\\
%\textbf{Add/Remove Folders} Add removes folders\\
%A facebook like application can then be written as follows:\
%Here follows the pseudo-code for an application that creates a Facebook wall, adds a status update to it, and then one picture.
%\begin{enumerate}
%\item \texttt{f=Create Feed}
%\item \texttt{t=Create Thread}
%\item bind(f,t);\\
%\item status=addTextToDB("This is a beautiful day");\\
%\item picture=addBlobToDB("/pictures/niceday.jpg");\\
%\item c1=addNetworkContent(status);\\
%\item c2=addNetworkContent(picture);\\
%\item addFeedEntry(f,c1);\\
%\item addFeedEntry(f,c2);\\
%\end{enumerate}

==> caching.tex <==
\subsection{Caching\label{lbl:cache}}
{\textcolor{red}{we have to show that: Feeds are distributed as a burst namely, most of people get the most of the data as they are created, and so for the update. I intend to use the dataset of -cite On the Evolution of User Interaction Viswanath- to prove this.
That the trusted peers do not share an object for more than a certain amount of time unless they received a fresh new update -or a certificate- for it. In few words, we want to be bandwidth efficient only when a big wave of downloads arrives not for random requests for old post (those can just refetch the content to the source). Using the minimum of exponential can prove that the path length has no real impact on efficiency because, since peers are committed to fetching the stream, there is an high chance that the content is just few hops away, AND THIS IS IMPORTANT ON A DHT YOU HAVE THE SAME PATH STRETCH BUT SINCE CONTENT IS EVENLY DISTRIBUTED THE PROBABILITY OF FINDING IT HALFWAY IS RATHER LOW. However, a more accurate model should be used, I found a paper from Kleinrock Tewari but I did not have time to finish reading it. The reason why content should NOT be cached for too long is due to the cost of fetching the Thread Update Stream. We might want to consider making an optimization model that given the reduces the unsafe time window to the minimum given the desired QoS}}

==> contribution.tex <==
`\section{Contribution\label{lbl:cont}}
This proposes an open infrastructure to decentralize the distribution of social data whilst enforcing user's privacy. \\
WARP allows to disseminate social data in an ICN fashion, leaving to the user the opportunity of deciding the right tradeoff between performance, security and control on his own data. The protocol is based a hierarchical name resolver to facilitate routing without lacking information about users' activities. \\
Data security is enforced using a combination of symmetric cryptography and Attribute Based Encryption (ABE) similarly to what is done in \cite{decent, easier} but with the only difference that WARP does not depend and proxies because for content updates. \\
Content updates are taken care of by implementing a two-way agreement between the producer of the original content and the producer of the update, namely, assuming the case of a comment on a facebook post, the first will agree to link the content update to his facebook wall as long as the second gives a signed certificate of what its comment contains and what the name of the data is. By creating this link, the owner of the wall prevents two problems, first, it links only comments that it consider appropriate and reputable, second, it certifies to his audience that the have not been compromised afterwards; at the same time the content update is bound with its actual producer which will also be responsible for its distribution. It is important to remark, that content updates are distributed at the same way of any other content and therefore they will be fetched either from their producer or from any cached copy in the network.\\
Instead of implementing a key-revocation protocol, whenever security policies change, cached objects are deleted, or substituted with a newly encrypted version. This is made possible by using control channels, named \textit{thread updates} which are used for delivering commands to content distributors. Note that thread updates are content at the very same way of normal data and therefore are routed, requested and even cached (only by distributors).\\ 
It is important to remark that we enforce caching to take care of the bursty nature of content requests -cite-, rather than long term data distribution. 









==> motivation.tex <==
\section{Motivation}
We aforementioned the issue of ownership of the data, at the current moment users do not maintain possess of the content that they upload on the OSNs servers -cite, and in the past there have also been cases of personal data sold without the consent of the users.
Moreover, by monitoring and analyzing topics and trends in people's shared content private companies can pitch their advertisement campaigns in order to deliver their message more effectively -cite-, while this process can be, arguably, considered transparent one could argue that the user should give an explicit consent before his data are read and processed. In this paper we aim at proposing an architecture that does not stops companies from making money with the social network, our idea is to prevent them to access to the user data without the explicit consent of the user. However, even when the user does not grant access to the data OSNs must be given the chance of selling their product with profit as an application that gives a contour to the social data. Let us, for instance, consider Facebook, at the current moment the "Facebook application" is a software runs on their servers the end user chooses how to interface to it, such as via a web-browser or a mobile application, in other words data are only generated at the source and then moved to Facebook that manages and distributes them. We want to reverse this scheme in an ICN fashion by having a Facebook application running on the source of the data, i.e. the user device, the application must have the duty of collecting the data from the user, whatever this are, and pass them to the WARP framework that takes care of encrypting them and distribute them to the network as a authenticated source. Note that this does not imply that Facebook cannot distribute the data anymore, for instance to improve the performance or offering the service in change of showing their advertisement, it only guarantee to the user that his data will not be accessible unless he decides to grant to Facebook the right of doing it. Our ultimate goal is to show that, with minor changes, ICN does this by-design, and that additionally it is possible to use WARP to build a shared social infrastructure as an overlay of the current Internet that is able t serve both the interests of OSNs and the rights of the users.
Whilst privacy is a critical matter when dealing with social data, it is not the only issue that a distributed social infrastructure could solve, for instance, recent events -cite- of defamatory campaigns over Twitter opened a debate  whether there should be a direct mapping between online users and individuals so that people have to take responsibilities for their actions, indeed having a direct mapping between content producer and data could help in this sense.
The same principle holds for aggregated statistics and surveys, websites gather feedback from their users about content, such as video articles etc, and then publish the results for everyone to see, however there is not a real way for the user to verify whether the results actually reflects reality because everything is based on the website reputation and the "likes" or "dislikes" are not signed by the users, furthermore there users can be fake and people can vote twice\footnote{There are indeed cases wherein anonymity should be enforced, for instance when discussing political views or delicate topics in general. Those cases are obviously not those we are referring to.}. By having this feedback signed and available as content over the network allows any users of the network to autonomously run a statistical test and verify the reliability of the statistic within his own interval of confidence, validating at the same time both the feedback statistics and the honesty of the website.


==> protocol_old.tex <==
\section{Protocol\label{sec:protocol}}
\subsection{Protocol Messages}
As discussed in Section \ref{sec:related}, ICN protocols generally use two types of messages, requests and data. WARP introduces two new of messages: \textbf{\textit{RESOLVE}} and \textbf{\textit{NOTIFY}}. \\
A \textbf{RESOLVE} message is used to obtain a list of distributors for a given folder, this type of query can be answered authoritatively only by the producer of the content or a distributor for a parent folder. In other words, considering the name \texttt{x.y/folder1/folder2/name1}
a butler that does not know a distributor for \texttt{x.y/folder1/folder2/} can obtain a list of distributors by sending a query to the butler \texttt{x.y} or any distributor for \texttt{x.y/folder1/}. This far we have not mentioned how to resolve machine addresses, generally speaking we do not consider this a real problem since both butlers and distributors rely on the IA to certify their identity, as long as the identity is associated with a domain name the name can be resolved using the normal DNS infrastructure.\\  
\textbf{NOTIFY} messages are one of the core ideas of WARP they are sent by a butler to another to inform that a content has been created. They are fundamental to implement common functionalities - such as comments, re-post, likes and re-tweets - since in WARP a network object cannot be modified by anybody that is not its producer. By design, content aggregation is operated at the application level rather than at the storage level namely, assuming the case of Alice adding a post on her Facebook wall and Bob commenting on it, in WARP there would be three distinct objects. Alice's post, Bob's comment and Alice's link to Bob's comment. A notify message contains a content-name, a signed checksum of the related data and an application identifier that says which application has generated the content.
\subsection{Thread Updates}
TUs are implemented as any other feed in the WARP network with the only difference that they deliver commands to caches.
Every network object is associated to a TU and carries a pointer to the latest object of the feed at the time it was created. Ideally content that are in the same TU should belong together so that for instance a comment belongs to the thread of the original post. However, we did not want to leave this kind of freedom to the developer and therefore we are using the following convention. Each folder has is monitored by its own TU, however, since TUs are also content and can be monitored at the same way each TU is monitored by the TU of its parent folder. This allows the distributors to have a finer control of what TUs to follow, for instance if a cloud service is distributing the entirety of a user's data it can follow a single thread for the user, differently if it is only distributing his photo album it will monitor only the folder containing its pictures.\\
The commands that a distributor receives from a TU are the following:\\
\textbf{ADD(X)} X has been create. The distributor can decide whether to prefetch X or not. \\  
\textbf{DELETE(X)} X must be purged from the cache and never distributed again.\\
\textbf{UPDATE(X,Y)} X has been updated with Y. The distributor must purge X, and can decide whether to download Y or not.  \\
\textbf{CUT(X,Y,X',Y')} A feed has been cut from X to Y. All the objects in between must be purged from the cache, the distributor can decide whether to download X' and Y' to merge the remaining pieces.\\
For our future work we are considering implementing a command that distributes only a differential of an updated object containing renewed version of the secret key and a new signature, however there are security issues to take into account and we do not consider it for the moment.
\subsection{Fetching of data}
Butlers and distributors maintain a routing table to direct their request. Each entry of the routing table contains a folder, a distributor and the expiration of the content. New requests that do not match any entry of the table trigger the butler to resolve the name and add a new entry to the routing table. 
\subsection{Serving Data}
In the generic ICN architecture whenever a cache, or a router, is requested for a content it verifies if there is a copy in its storage otherwise it forwards the request to another cache to obtain a copy. Whenever the copy arrives it can decide whether this should be cached or not. WARP approach is slightly different since it must consider TUs. The logic for serving an incoming request for a content $R$  follows:\\
{
\textbf{1.} If R is not in the Content Store go to 6\\
\textbf{2.} Is the content stale? if yes go to 6\\
\textbf{3.} Have $T_R$ been checked recently? if yes, go to 7\\
\textbf{4.} Fetch $T_R$\\
\textbf{5.} Is the content still valid? if yes, go to 7\\
\textbf{6.} Fetch R\\
\textbf{7.} Serve Request \\
\textbf{8.} Is R popular? if not go to end.\\
\textbf{9.} Is the $T_R$ alr? if yes go to 7\\
\textbf{10.} Start follow $T_R$\\
\textbf{11.} Cache R \\
}
\subsection{Continuous Polling}
A possible attack that can tamper the cache control mechanism of WARP is \textbf{continuous polling}: a malicious butler generates requests at a high frequency so that it can receive every version of a content before being excluded from the followers.
This problem can be solved on the distributor side by implementing a \textit{Request Ban Window} (RBW), for every open connection distributors keep track of when each a butler is allowed to send a new request, if a request arrives before then they do not serve it. 
Also, whenever they receive a request from the butler they update the RBW to the maximum between its current value and the value of a function:
$$T_{RBW}(t) = \mbox{current time} + \left\{
\frac{fail(t,\delta)}{1 + succ(t,\delta)}\cdot \delta \\
\right.$$
where $fail(t,delta)$ and $succ(t,\delta)$ respectively are the number of failed and successful requests that a butler has sent in the latest time window of length $delta$. Note that $T_{RBW}(t)$ scales the RBW $\delta$ according to the \textit{hit-ratio} of the butlers request, if the requests are mostly successful - i.e. there is a burst of data to download - the butler is allowed to send requests faster, differently, if the requests are unsuccessful the time window grows.
Butlers that respect the suggested inter-request time will never have their requests rejected whereas butlers that do not will delay their opportunity of downloading.


==> related.tex <==
\section{Related Work}
`
\subsection{Decentralized Social Networks}

==> sn_arch_img.tex <==
\begin{figure*}[t!]
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=\linewidth]{img/arch_cur.jpg}
\subcaption{}
\label{fig:figure2}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=\linewidth, height= 4cm]{img/arch_new.jpg}
\subcaption{}
\label{fig:figure1}
\end{minipage}
\caption{{\scriptsize }}
\end{figure*}
